Human-Centred Learning Analytics and AI in Education: a Systematic Literature Review

The rapid expansion of Learning Analytics (LA) and Artificial Intelligence in Education (AIED) offers new scalable, data-intensive systems but also raises concerns about data privacy and agency. Excluding stakeholders -- like students and teachers -- from the design process can potentially lead to mistrust and inadequately aligned tools. Despite a shift towards human-centred design in recent LA and AIED research, there remain gaps in our understanding of the importance of human control, safety, reliability, and trustworthiness in the design and implementation of these systems. We conducted a systematic literature review to explore these concerns and gaps. We analysed 108 papers to provide insights about i) the current state of human-centred LA/AIED research; ii) the extent to which educational stakeholders have contributed to the design process of human-centred LA/AIED systems; iii) the current balance between human control and computer automation of such systems; and iv) the extent to which safety, reliability and trustworthiness have been considered in the literature. Results indicate some consideration of human control in LA/AIED system design, but limited end-user involvement in actual design. Based on these findings, we recommend: 1) carefully balancing stakeholders' involvement in designing and deploying LA/AIED systems throughout all design phases, 2) actively involving target end-users, especially students, to delineate the balance between human control and automation, and 3) exploring safety, reliability, and trustworthiness as principles in future human-centred LA/AIED systems.

==> sections/hcai-table.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|p{7.5cm}|p{7.5cm}|}
        \hline
        & \multicolumn{3}{c|}{Computer Automation (CA)} \\ 
        \cline{2-4}
        & & \centering LOW CA & \multicolumn{1}{c|}{HIGH CA} \\
        \cline{3-4}
        & & \centering \textbf{Q2}: High HC and Low CA ($n=33$) & \multicolumn{1}{c|}{\textbf{Q4}: High HC and High CA ($n=49$)} \\
        & HIGH HC &
        %Q2 
\citenum{topaliSupportingInstructorsDesign2022,michosInvolvingTeachersLearning2020,readParticipatoryDesignDevelopment2012,vinellaFormingTeamsLearners2022};
\citenum{tsaiChartingDesignNeeds2022,oliver-quelennecAdaptingLearningAnalytics2022,pishtariMultistakeholderPerspectiveAnalytics2021,chattiHowDesignEffective2020,Ahn2021Apr};
\citenum{treasure-jonesHowStudentsWant2018,fernandez-nietoClassroomDandelionsVisualising2022, muslimRuleBasedIndicatorDefinition2016,mangaroskaGazeInsightsDebugging2018,wangHowDoesOrder2019};
\citenum{cukurovaInteractionAnalysisOnline2017,longMotivationalDesignIntelligent2015,muldnerDesigningTangibleLearning2013, ternbladPreschoolersGameSystem2018,desilvaInstitutionalAnalyticsAgenda2022};
\citenum{rappScalingAcademicWriting2018,shuteDesignDevelopmentTesting2021,tenorioExploringDesignConcepts2022,hosseiniImprovingEngagementProgram2020,alboKnowledgeBasedDesignAnalytics2022};
\citenum{rodriguesHowPersonalizationAffects2023,easterdayDesigningCrowdcritiqueSystems2017, martinezImpactUsingLearning2020, mcneillAsymptomaticsZombiesVisualizationbased2023a};
\citenum{camaraolimPeriodicFableDiscovery2023a, jeongAutomataStageARMediatedCreativity2023a, crainVisualizingTopicsOpinions2022a, shreinerInformationWonJust2022a, huITalkISeeParticipatory2022a}
& 
        % Q4
        \citenum{conijnHowProvideAutomated2020,shibani2022questioning,ocumpaughGuidanceCounselorReports2017};
        \citenum{holstein2019Codesign,tissenbaumSupportingClassroomOrchestration2019,kangARMathAugmentingEveryday2020,labonte-lemoyneBusinessIntelligenceSerious2017,liaqatCollaboratingMatureEnglish2021};
        \citenum{olsenDesigningCoOrchestrationSocial2021,jonssonCrackingCodeCocoding2022,wangCoDesigningAIAgents2022,zhangStoryBuddyHumanAICollaborative2022};
        \citenum{nazaretskyEmpoweringTeachersAI2022,pozdniakovQuestiondrivenDashboardHow2022,conijnHowProvideAutomated2020,dollinger2019working,dimitriKeepMeLoop2022};
        \citenum{alevenDashboardSupportTeachers2022,yangTechnologyEcosystemOrchestrating2022,limImpactLearningAnalytics2021,martinez-maldonadoLATUXWorkflowDesigning2015,fernandez2022beyond};
        \citenum{gibsonReflectiveWritingAnalytics2017,dequinceyStudentCentredDesign2019,al-doulatMakingSenseStudent2020,lalleImpactStudentIndividual2017,borjiginTeachableAgentsIntrinsic2015,headToneWarsConnectingLanguage2014,ruiz-callejaInfrastructureWorkplaceLearning2019};
        \citenum{rodriguez-trianaAdaIblLessons2021,khosraviRiPPLECrowdsourcedAdaptive2019,chavanTcherlyTeacherFacingDashboard2022,vannaprathipIntelligentTutoringSurgical2022,hanMakingFAQChatbots2022,sulemanNewPerspectiveNegotiationBased2016};
        \citenum{khachatryanReasoningMindGenie2014,schulzTutoringSystemSupport2022,tegosConfigurableConversationalAgent2014,maGlanceeAdaptableSystem2022, luoResearchDesignProjectbased2022a, alfredoThatStudentShould2023a, oogeSteeringRecommendationsVisualising2023a};
        \citenum{satoGroupnamicsDesigningInterface2023a, leePrototypingSpatialSkills2022a, bonnatDigitalCompanionMonitor2022a, leeHumanCentricAutomatedEssay2023a,hutchinsUsingTeacherDashboards2023a}
        \\
        \cline{2-4}
        & & \centering\textbf{Q1}: Low HC and Low CA ($n=12$) & \multicolumn{1}{c|}{\textbf{Q3}: Low HC and HIGH CA ($n=10$)}\\
        % Q1
         \multirow{-9}{*}{\rotatebox{-90}{Human Control (HC)}} & LOW HC & 
        \citenum{vezzoliInspirationCardsWorkshops2020,echeverriaCollaborationTranslucenceGiving2019,eradzeContextualisingLearningAnalytics2020,fernandez-nietoModellingSpatialBehaviours2021,challcoCanOntologiesSupport2020,kivimakiCurricularConceptMaps2019,nguyenMixedmethodStudyHow2020};
        \citenum{sorenyCodesignDigitalLearning2022a, boatengPreServiceTeachersPerspectives2022a, garcia-ruizParticipatoryDesignSonification2022a, zwolinskiExtendedRealityEducation2022a,bishopDesignUsabilityAvatarBased2022a}
        &  
        %Q3 
    \citenum{ekstromDualRoleHumanoid2022,shardlowCollaborativeAugmentationSimplification2022,assimRemoteTeachingCOVID192021,zhouInvestigatingStudentsExperiences2021,weigandHCD3AHCDModel2021,huttBreakingOutLab2021,ochoaControlledEvaluationMultimodal2020,wilsonAutomatedFeedbackAutomated2021,santosGoalOrientedVisualizationsActivity2012};
    \citenum{kimExplainWhatTreemap2023a}
        \\
        \hline
    \end{tabular}
    \caption{
    Reviewed human-centred LA/AIED papers distributed across the four HCAI quadrants of human control and computer automation. The number is a unique identifier according to its ordinal position in references. Sorted reference details are also available in Appendix A, Table \ref{table:appendix-reference}}
    \label{tab:hcai-results}
\end{table}
